AdaWCT: Adaptive Whitening and Coloring Style Injection

Adaptive instance normalization (AdaIN) has become the standard method for style injection: by re-normalizing features through scale-and-shift operations, it has found widespread use in style transfer, image generation, and image-to-image translation. In this work, we present a generalization of AdaIN which relies on the whitening and coloring transformation (WCT) which we dub AdaWCT, that we apply for style injection in large GANs. We show, through experiments on the StarGANv2 architecture, that this generalization, albeit conceptually simple, results in significant improvements in the quality of the generated images.

==> prenorm.tex <==
%!TEX root = main.tex
\section{Pre-normalization}
\label{app:pre-normalization}

\todo{Put in supp. mat? Not sure it's allowed @ ICIP... }

La démonstration suivante consolide la justification de cette pré-normalisation. Notons ici
$\mathbf{\Sigma} \in \mathbb{R}^{a \times a}$ la matrice d'intérêt et $\mathbf{I} \in \mathbb{R}^{a
\times a}$ une matrice identité alors $\mathbf{A} = \mathbf{I} - \frac{\mathbf{\Sigma}}{\left
\|\mathbf{\Sigma} \right \|_{F}}$ à des fins de simplification. La condition de convergence dans le
cas $p=2$ correspond alors à $\left \|\mathbf{A} \right \|_{2} < 1$.

Pour toute matrice $\mathbf{B} \in \mathbb{R}^{b \times b} $ ayant des valeurs propres $\lambda_i$
ainsi que des vecteurs propres $\nu_i$ pour $i \in \{1, \dotsc, b\}$, pour tout scalaire $c$ alors
$\lambda_b + c$ correspond aux valeurs propres de la matrice résultantes de la somme des matrices
$\mathbf{B} + c\mathbf{I}$.


Suivant ce résultat, il est possible de conclure que les valeurs propres de $\mathbf{A}$
correspondent à

\begin{equation}
  \label{eqn:A_eigenvals}
  \lambda_i(\mathbf{A}) = 1 - \frac{\sigma_{i}(\mathbf{\Sigma})}{\sqrt{\sum_{j}\sigma_{j}(\mathbf{\Sigma})^{2}}},
\end{equation}

pour $i \in \{1, \dotsc, a\}$.

La matrice \textbf{A} étant symétrique, ses valeurs singulières correspondent à $\sigma_i = \left |
\lambda_i  \right |$ et donc 
\begin{equation}
  \label{eqn:A_singular_vals}
  \sigma_i = \left |1 - \frac{\sigma_{i}}{\sqrt{\sum_{j}\sigma_{j}^{2}}}  \right |.
\end{equation}

Considérant la norme matricielle $\left \|\mathbf{A} \right \|_{2} = \sigma_{max}(\mathbf{A})$, le
critère de convergence $\left \|\mathbf{A} \right \|_{2} < 1$ peut être exprimé $\sigma_{max}(\mathbf{A}) < 1$.

Étant donné que l'on cherche la valeur singulière maximale de la matrice $\mathbf{A}$ correspondant
à la différence de $1 - \frac{\sigma_{a}}{\sqrt{\sum_{j}\sigma_{j}^{2}}}$, $\sigma_{a}$ sera par
conséquent la plus petite valeur singulière (a-ième valeur singulière) de la matrice
$\frac{\mathbf{\Sigma}}{\left \|\mathbf{\Sigma} \right \|_{F}}$.

Il est possible d'observer que la plus grande valeur singulière de la matrice $\mathbf{A}$ correspond à
\begin{equation}
  \label{eqn:plus_grande_val_sing}
  \left |1 - \frac{\sigma_{a}}{\sqrt{\sum_{j}\sigma_{j}^{2}}}  \right | < 1.
\end{equation}

Le résultat de cette équation est toujours inférieur à 1 puisque la division d'une des valeurs
singulière par la somme de toutes les valeurs singulière produit un résultat inférieur à 1. Cette
conclusion permet d'assurer un respect de la condition de convergence. De plus, l'ajout de
l'estimateur de contraction $\epsilon$ garantie que le résultat ne puisse égaler 1 et donc briser la
condition de convergence.
